sGUARD: Towards Fixing Vulnerable Smart Contracts Automatically

Smart contracts are distributed, self-enforcing programs executing on top of blockchain networks. They have the potential to revolutionize many industries such as financial institutes and supply chains. However, smart contracts are subject to code-based vulnerabilities, which casts a shadow on its applications. As smart contracts are unpatchable (due to the immutability of blockchain), it is essential that smart contracts are guaranteed to be free of vulnerabilities. Unfortunately, smart contract languages such as Solidity are Turing-complete, which implies that verifying them statically is infeasible. Thus, alternative approaches must be developed to provide the guarantee. In this work, we develop an approach which automatically transforms smart contracts so that they are provably free of 4 common kinds of vulnerabilities. The key idea is to apply runtime verification in an efficient and provably correct manner. Experiment results with 5000 smart contracts show that our approach incurs minor run-time overhead in terms of time (i.e., 14.79%) and gas (i.e., 0.79%).

==> sections/appendices.tex <==
\appendices

\section{Operational  semantics  of  Ethereum  opcode}
\label{fstapp}

The semantics of opcodes are shown in Figure~\ref{fig:op} in form of execution rules, each of which is associated with a specific opcode. Each rule is composed of multiple conditions above the line and a state change below the line. The state change is read from left to right, i.e., the state on the left changes to the state on the right if the conditions above the line are satisfied.

Most of the rules are self-explanatory and thus we skip the details and refer the readers to~\cite{9152785}. It is worth mentioning how external calls are abstracted in our semantic model. Given an external function call (i.e., opcode \term{CALL}), the execution temporarily switches to an execution of the invoked contract. The result of the external call, abstracted as $res$, is pushed to the stack. %\sjsay{It is not clear how this modeling works, for instance, to capture behaviors such as reentrancy.}

\begin{figure*}[t]
\begin{frameit}
\small\centering
$$
\infer[\term{STOP}]
{
(pc,S,M,R) \nxt \lst
}
{
\begin{array}{c}
\end{array}
}
\quad
\infer[\term{POP}]
{
(pc,S,M,R) \nxt (pc+1,S_1,M,R)
}
{
\begin{array}{c}
S_1,x = S.pop()
\end{array}
}
\quad
\infer[\term{UNARY-op}]
{
(pc,S,M,R) \nxt (pc+1,S_2,M,R)
}
{
\begin{array}{c}
S_1,x = S.pop()~~z = op(x)~~S_2 = S_1.push(z)
\end{array}
}
$$
$$
\infer[\term{BINARY-op}]
{
(pc,S,M,R,pc) \nxt (pc+1,S_3,M,R,pc+1)
}
{
\begin{array}{c}
S_1,x = S.pop()~~~~S_2,y = S_1.pop()\\z = op(x,y)~~~~S_3 = S_2.push(z)
\end{array}
}
\quad
\infer[\term{TERNARY-op}]
{
(pc,S,M,R) \nxt (pc+1,S_4,M,R)
}
{
\begin{array}{c}
S_1,x = S.pop()~~S_2,y = S_1.pop()~~S_3,m = S_2.pop()\\z = op(x,y,m)~~~~S_4 = S_3.push(z)
\end{array}
}
$$
$$
\infer[\term{MLOAD}]
{
(pc,S,M,R) \nxt (pc+1,S_2,M,R)
}
{
\begin{array}{c}
S_1,p = S.pop()~~v = M[p]~~S_2 = S_1.push(v)
\end{array}
}
\quad
\infer[\term{MSTORE}]
{
(pc,S,M,R) \nxt (pc+1,S_2,M_1,R)
}
{
\begin{array}{c}
S_1,p = S.pop()~~S_2,v = S_1.pop()~~M_1 = M[p \leftarrow v]
\end{array}
}
$$
$$
\infer[\term{SLOAD}]
{
(pc,S,M,R) \nxt (pc+1,S_2,M,R)
}
{
\begin{array}{c}
S_1,p = S.pop()~~v = R[p]~~S_2 = S_1.push(v)
\end{array}
}
\quad
\infer[\term{SSTORE}]
{
(pc,S,M,R) \nxt (pc+1,S_2,M,R_1)
}
{
\begin{array}{c}
S_1,p = S.pop()~~S_2,v = S_1.pop()~~R_1 = R[p \leftarrow v]
\end{array}
}
$$
$$
\infer[\term{DUP-i}]
{
(pc,S,M,R) \nxt (pc+1,S_1,M,R)
}
{
\begin{array}{c}
v = S.get(i)~~S_1 = S.push(v)
\end{array}
}
~~
\infer[\term{SWAP-i}]
{
(pc,S,M,R) \nxt (pc+1,S_2,M,R)
}
{
\begin{array}{c}
v_0 = S.get(0)~~v_i = S.get(i)~~S_1 = S[0 \leftarrow v_i]~~S_2 = S_1[i \leftarrow v_0]
\end{array}
}
$$
$$
\infer[\term{JUMPI-t}]
{
(pc,S,M,R) \nxt (lbl,S_2,M,R)
}
{
\begin{array}{c}
S_1,lbl = S.pop()~~S_2,c = S_1.pop()~~c \neq 0
\end{array}
}
~~
\infer[\term{JUMPI-f}]
{
(pc,S,M,R) \nxt (pc+1,S_2,M,R)
}
{
\begin{array}{c}
S_1,lbl = S.pop()~~S_2,c = S_1.pop()~~c = 0
\end{array}
}
$$
$$
\infer[\term{JUMP}]
{
(pc,S,M,R) \nxt (lbl,S_1,M,R)
}
{
\begin{array}{c}
S_1,lbl = S.pop()
\end{array}
}
\quad\quad\quad
\infer[\term{CALL}]
{
(pc,S,M,R) \nxt (pc+1,S_1,M,R)
}
{
\begin{array}{c}
res = call()~~S_1 = S.push(res)
\end{array}
}
$$
$$
\infer[\term{SHA3}]
{
(pc,S,M,R) \nxt (pc+1,S_3,M,R)
}
{
\begin{array}{c}
S_1,p = S.pop()~~S_2,n = S_1.pop()~~v = sha3(M[p,p+n])~~S_3 = S_2.push(v)
\end{array}
}
$$
\end{frameit}
\caption{Operational semantics of Ethereum opcodes. $pop$, $push$, and $get$ are self-explanatory stack operations. $m[p \leftarrow v]$ denote an operations which returns the same stack/mapping as $m$ except that the value of position/key $p$ is changed to $v$.
%The initial state of any execution is $<\emptyset, \emptyset, R_0, 0>$ in which the stack and the memory are empty, the storage is like when the transaction is invoked, and the program counter is 0. 
Rule \term{UNARY-op} (\term{BINARY-op}, \term{TERNARY-op}) applies to all unary (binary, ternary) operations; rule \term{DUP-i}, applies to all duplicate operations; and rule \term{SWAP-i} applies to all swap operations. %The 3 rules \term{UNARY-op}, \term{BINARY-op}, and \term{TERNARY-op} are concretized by setting the specific operation which will be applied in the execution of the rules. Similarly, the 2 rules \term{DUP-i} and \term{SWAP-i} are concretized by setting the value of the variable $i$, which can be from 1 to 16. 
%The control flow can be changed by 3 rules: \term{JUMP-T}, \term{JUMP-F} and \term{JUMP}.
}\label{fig:op}
\end{figure*}

% \section{Second Appendix}

% \begin{table*}[h]
% {\scriptsize
% \begin{tabular}{|l|l|}
% \hline
% Rule & Opcodes \\
% \hline
% \term{STOP} & \texttt{SELFDESTRUCT}, \texttt{REVERT}, \texttt{INVALID}, \texttt{RETURN}, \texttt{STOP}  \\ \hline
% \term{POP} & \texttt{POP} \\ \hline
% \term{UNARY-op} & \texttt{NOT}, \texttt{ISZERO}, \texttt{CALLDATALOAD}, \texttt{EXTCODESIZE}, \texttt{BLOCKHASH}, \texttt{BALANCE}, \texttt{EXTCODEHASH} \\ \hline
% \term{BINARY-op} & \texttt{ADD}, \texttt{MUL}, \texttt{SUB}, \texttt{DIV}, \texttt{SDIV}, \texttt{MOD}, \texttt{SMOD}, \texttt{EXP}, \texttt{SIGNEXTEND}, \texttt{LT}, \texttt{GT}, \texttt{SLT}, \texttt{SGT}, \texttt{EQ}, \texttt{AND}, \texttt{OR}, \texttt{XOR}, \texttt{BYTE}, \texttt{SHL}, \texttt{SHR}, \texttt{SAR} \\ \hline
% \term{TERNARY-op} & \texttt{ADDMOD}, \texttt{MULMOD}, \texttt{CALLDATACOPY}, \texttt{CODECOPY}, \texttt{RETURNDATACOPY} \\ \hline
% \term{MLOAD} & \texttt{MLOAD} \\ \hline
% \term{MSTORE} & \texttt{MSTORE}, \texttt{MSTORE8} \\ \hline
% \term{SLOAD} & \texttt{SLOAD} \\ \hline
% \term{SSTORE} & \texttt{SSTORE} \\ \hline
% \term{DUP-i} & \texttt{DUP1}$\cdots$\texttt{DUP16}\\ \hline
% \term{SWAP-i} & \texttt{SWAP1}$\cdots$\texttt{SWAP16} \\ \hline
% \term{JUMPI-t/JUMPI-f} & \texttt{JUMPI}\\ \hline
% \term{JUMP} & \texttt{JUMP}\\ \hline
% \term{CALL} & \texttt{STATICCALL}, \texttt{CALL}, \texttt{CALLCODE}, \texttt{CREATE}, \texttt{CREATE2}, \texttt{DELEGATECALL}, \texttt{SELFDESTRUCT} \\ \hline
% \term{SHA3} & \texttt{SHA3} \\ \hline
% \end{tabular}
% }
% \caption{The opcodes according to each rule}
% \label{tbl:op}
% \end{table*}

==> sections/code-fig.tex <==
\begin{figure}[t]
\centering
\small
\[
\begin{array}{rcl}
prog  & ::= & data^* func^* \\
data  & ::= & type~\textrm{\bf{id}} \\
func  & ::= & {\textrm{\bf{id}}?~{\bf{payable}}?~(data^*)~\{stmt^*\}} \\
stmt  & ::= &  \textrm{\bf{id}}~{:=}~expr ~|~ \textrm{\bf{id}}.\textrm{\bf{id}}~{:=}~expr ~|~ \textrm{\bf{id}}[expr]~{:=}~expr ~|~ \\           
      & &        \textrm{\bf{if}}~(expr)~\textrm{\bf{then}}~{\{stmt_1^*\}}~\textrm{\bf{else}}~{\{stmt_2^*\}} ~|~ \textrm{\bf{while}}~(expr)~\textrm{\bf{do}}~{\{stmt^*\}} ~|~\\
      & &        \textrm{\bf{throw}} ~|~ \textrm{\bf{suicide}}(addr) ~|~ call \\
call  & ::= & addr.opt^*\textrm{\bf{call}}(expr^*) ~|~ addr.opt^*\textrm{\bf{delegatecall}}(expr^*) ~|~ addr.opt^*\textrm{\bf{id}}(expr^*) \\
      & &        addr.{\bf{send}}(k) ~|~ addr.{\bf{transfer}}(k) \\
opt   & ::= & \textrm{\bf{gas}}(k) ~|~ \textrm{\bf{value}}(k) \\
expr  & ::= &  k ~|~ \textrm{\bf{id}} ~|~ \textrm{\bf{id}}.\textrm{\bf{id}} ~|~ \textrm{\bf{id}}[expr] ~|~ expr_1~op_b~expr_2 ~|~ op_u~expr
\end{array}
\]
\caption{A core language}\label{code-fig}
\end{figure}


==> sections/semantics.tex <==
\newcommand{\term}[1]{\textsc{#1}}
\newcommand{\conf}[1]{\langle #1 \rangle}
\newcommand{\eval}[1]{[ #1 ]}
\newcommand{\ctx}{\Gamma}
\newcommand{\nxt}{\leadsto}
\newcommand{\lst}{\Box}
\newcommand{\wrong}{\blacksquare}
\newcommand{\gas}{\mathcal{G}}
\newcommand{\defi}{\stackrel{\triangle}{=}}
\newcommand{\prim}{\mathsf{basic}}
\newcommand{\kil}{\times}
\newcommand{\hide}[1]{}
\newcommand{\env}{\mathcal{E}}
\newcommand{\bal}{\mathcal{B}}
\newcommand{\sife}[3]{{\bf{if}}~#1~{\bf{then}}~#2~{\bf{else}}~#3}
\newcommand{\swhile}[2]{{\bf{while}}~#1~{\bf{do}}~#2}
\newcommand{\fback}{{\bf{fallback}}}

Having our core language described previously in~\S\ref{sub:corelang}, we proceed to establish a light-weight operational semantics for it in Fig.~\ref{fig:op}. Before going into the details, we would like to introduce several notations that are useful for the later semantics construction. Our main ledger $\ctx$ is a mapping between addresses and contracts, while each contract is modeled by a triple $(\sigma,\textit{bal},\mathcal{C})$ where $\sigma$ is the contract persistent memory, $\textit{bal}$ is the contract balance, and $\mathcal{C}$ holds the contract source code together with its address. Each transaction $T$ is a triple $(c,g,\sigma_T)$ that consists of the executed code/function $c$, the gas stipend $g$, and the \emph{transaction context} $\sigma_T$ which contains all relevant information such as time stamp, addresses of the sender/receiver, input data, \emph{etc}. For the step relation, we use two separate types of configuration: the transaction configuration $\conf{\ctx,\mathcal{T}}$ represented by a pair of ledger $\ctx$ and transaction list $\mathcal{T}$; and the contract configuration $\conf{\conf{c,\sigma_A,\mathcal{C}},g,\ctx}$  consisting of the running code $c$, an auxiliary environment $\sigma_A$ for temporary variables, memory allocations, as well as static information of the current transaction, the callee contract $\mathcal{C}$, the gas stipend $g$, and the main ledger $\ctx$. Furthermore, the triple $\conf{c,\sigma_A,\mathcal{C}}$ in the transaction configuration serves as the activation record to keep track of the control flow as well as to handle context switching for function calls. For the purpose of bookkeeping, we allow two more symbols to be added into the running code $c$ inside the activation record: $\lst$ which means the code is executed successfully, and $\wrong$ to signal that an exception has been occurred. To specify the changes in the main ledger, we use the the following notations: $\ctx[\textit{addr}_1 \stackrel{v}{\rightarrow} \textit{addr}_2]$ represents the ledger after transferring $v$ ethers from $\textit{addr}_1$ to $\textit{addr}_2$ in $\ctx$, and $\ctx[\textit{addr} \leftarrow \mathsf{None}]$ means that the contract at address $\textit{addr}$ is removed from $\ctx$. Also, multiple changes $t_1,\ldots,t_n$ over $\ctx$ can be simply expressed as $\ctx[t_1]\ldots[t_n]$. Lastly, we adapt the evaluation format $E \models \eval{\textit{expr}} = v$ which says that the expression $\textit{expr}$ is evaluated to the value $v$ under the context $E$.   

Our semantics is designed using a two-layer architecture: the transaction layer describing how the main ledger is updated per transaction, and the contract layer where the code of the corresponding contract is executed accordingly. At the transaction layer, the relation step is a pair of transaction configurations, \emph{e.g.} $\conf{\ctx,\mathcal{T}} \nxt \conf{\ctx',\mathcal{T}'}$; similarly the relation step at the contract level is defined as a pair of contract configurations, \emph{e.g.} $\conf{\conf{c,\sigma_T,\mathcal{C}},g,\ctx} \nxt \conf{\conf{c',\sigma',\mathcal{C}'},g',\ctx'}$. To ease the gas accounting which is usually done after compilation at the byte code level, we abstract away the gas usage for executing the contract code $c$ using an oracle function $\gas(c,g,\sigma_A,\ctx)$ so that we can query the gas usage of $c$ based on the code $c$ itself, the available gas $g$, the current auxiliary environment $\sigma_A$, and all the relevant information that can be found in the ledger $\ctx$. 

Given all the necessary definitions at hand, we are now ready to explain the meaning of each semantics rule in Fig.~\ref{fig:op}. The first two rules $\term{Succ}$ and $\term{Fail}$ narrate what happen at the transaction level. In detail, if the code $c$ is executed successfully at the contract level, \emph{i.e.} a contract configuration marked with $\lst$ can be reached, then the rule $\term{Succ}$ allows the ledger state to be updated accordingly. Otherwise, if an exception is raised and the contract configuration is marked with $\wrong$ then the rule $\term{Fail}$ is applied so that the whole transaction is reverted and the old ledger state will be used for the next transaction. Note that the initial auxiliary context $\sigma_A$ is set to be $\sigma_T$, the transaction context; also all static data recorded in $\sigma_T$ such as time stamp, sender address, \emph{etc}, will be propagated appropriately via the step relation and thus are accessible from $\sigma_A$ inside the activation record. The remaining rules describe how the step relation behaves at the contract level. The rule $\term{Gas}_\wrong$ exclusively handles cases where there is not enough gas to run the next statement in the contract code and thus an exception $\wrong$ is raised inside the activation record. Its counterpart rule $\term{Gas}$ is applied whenever the code $c$ is a \emph{basic statement}, \emph{e.g.} variable assignment, object creation, \emph{etc}, where the gas accounting is done according using $\gas$ and the rule's premise is simply the step relation of sequential machine. Several other rules such as $\term{Sk}$, $\term{Seq}$, $\term{Th}$, $\term{If}_\top$, $\term{If}_\bot$, $\term{Wh}_\top$, $\term{Wh}_\bot$ are standard in sequential semantics and thus self-explanatory; one major difference is that we need to compute the gas usage whenever checking boolean expressions inside conditional statements. The rule $\term{Sc}$ defines the behavior of the $\textit{addr}.{\bf{suicide}}$ function in which the remaining balance of the current contract $\mathcal{C}$ is sent to address $\textit{addr}$, followed by $\mathcal{C}$ being removed from the ledger $\ctx$. The two rules $\term{Call}$ and $\term{Call}_\wrong$ state the configuration changes when a function call happens: a gas stipend $g'$ and an ether amount $v$ from the contract balance are passed to $\textit{addr}$ to run the function $f$ with parameter $\bar{e}$, at the same time a context switching happens inside the activation record. If $f$ runs successfully and reaches a configuration marked with $\lst$ then the rule $\term{Call}$ allows the relevant balances to be updated accordingly. Otherwise if an exception occurs, the ledger state is reverted back to the moment before the function call. The two rules $\term{Tf}$ and $\term{Tf}_\wrong$ frame the behavior of the {\bf{send}} function, which, at a first glance, looks like a special case of {\bf{call}} where the $\fback$ function of the callee is called with a gas stipend of 2300. Nevertheless, the key difference is that the exception raised by {\bf{transfer}} is continuously propagated to the caller. The rule $\term{send}$ describing the behavior of {\bf{send}} as a special case of {\bf{call}} in which the $\textit{addr}.\fback$ function  is called given a gas stipend of 2300. Lastly, we have two rules $\term{Dc}$ and $\term{Dc}_\wrong$ for {\bf{delegatecall}}. The crucial dissimilarity between {\bf{delegatecall}} and {\bf{call}} is that the former uses the context of the caller whereas there is a context switching to the callee context for the latter. This distinction is expressed precisely in our rules by choosing the appropriate auxiliary context for the activation record.     
\begin{figure}[h]
$$
\infer[\term{Succ}]
{
\conf{\ctx,T::\mathcal{T}} \nxt \conf{\ctx',\mathcal{T}}
}
{
\begin{array}{c}
\ctx(\sigma_T.\textit{addr}_r) = (\sigma,\textit{bal},\mathcal{C})
\\
\conf{\conf{c,\sigma_T,\mathcal{C}},g,\ctx} \nxt \conf{\conf{\lst,\sigma',\mathcal{C}},g',\ctx'}
\end{array}
}~~~
\infer[\term{Fail}]
{
\conf{\ctx,T::\mathcal{T}} \nxt \conf{\ctx,\mathcal{T}}
}
{
\begin{array}{c}
\ctx(\sigma_T.\textit{addr}_r) = (\sigma,\textit{bal},\mathcal{C})
\\
\conf{\conf{c,\sigma_T,\mathcal{C}},g,\ctx} \nxt \conf{\conf{\wrong,\sigma_A',\mathcal{C}},g',\ctx'}
\end{array}
}$$
$$
\infer[\term{Gas}_\wrong]
{
\conf{\conf{c,\sigma_A,\mathcal{C}},g,\ctx} \nxt \conf{\conf{\wrong,\sigma_A,\mathcal{C}},g',\ctx'}
}
{
\gas(c,g,\sigma_A,\ctx) < 0
}~~~
\infer[\term{Gas}]
{
\conf{\conf{c,\sigma_A,\mathcal{C}},g,\ctx} \nxt \conf{\conf{\lst,\sigma_A',\mathcal{C}},g',\ctx'}
}
{
\begin{array}{c}
c \in \prim ~~~g' = \gas(c,g,\sigma_A,\Gamma) \geq 0
\\\conf{c,\sigma_A,\mathcal{C},\ctx} \nxt \conf{\lst,\sigma'_A,\mathcal{C},\ctx'}
\end{array}
}
$$
$$
\infer[\term{Th}]
{
\conf{\conf{{\bf{throw}};c,\sigma_A,\mathcal{C}},g,\ctx} \nxt \conf{\conf{\wrong,\sigma_A,\mathcal{C}},g,\ctx}
}
{}~~~
\infer[\term{Sk}]
{
\conf{\conf{\lst;c,\sigma_A,\mathcal{C}},g,\ctx} \nxt \conf{\conf{c,\sigma_A,\mathcal{C}},g,\ctx}
}
{}
$$
$$
\infer[\term{Seq}]
{
\conf{\conf{c_1;c_2,\sigma_A,\mathcal{C}},g,\ctx} \nxt
\conf{\conf{c_1';c_2,\sigma_A',\mathcal{C}},g',\ctx'}
}
{
\conf{\conf{c_1,\sigma_A,\mathcal{C}},g,\ctx} \nxt
 \conf{\conf{c_1',\sigma_A',\mathcal{C}},g',\ctx'}
}~~~
\infer[\term{Sc}]
{\begin{array}{c}
\conf{\conf{\textit{addr}.{\bf{suicide}};c,\sigma_A,\mathcal{C}},g,\ctx} \nxt
\\
 \conf{\conf{\lst,\sigma_A,\mathcal{C}},g,\ctx'}
\end{array}
}
{
\begin{array}{c}
\ctx[\mathcal{C}.\textit{addr}].\textit{bal} = b
\\
\ctx' = \ctx[\mathcal{C}.\textit{addr}  \xrightarrow{b} \textit{addr}][\mathcal{C}.\textit{addr} \leftarrow \mathsf{None}]
\end{array}
}
$$
$$
\infer[\term{If}_\top]
{
\begin{array}{c}
\conf{\conf{\sife{b}{c_1}{c_2},\sigma_A,\mathcal{C}},g,\ctx} \nxt 
\\
\conf{\conf{c_1,\sigma_A,\mathcal{C}},g',\ctx}
\end{array}
}
{
\begin{array}{c}
g' = \gas(b,g,\sigma_A, \ctx) \geq 0
\\
\ctx,\sigma_A \models \eval{b} =\top
\end{array}
}~~~
\infer[\term{If}_\bot]
{
\begin{array}{c}
\conf{\conf{\sife{b}{c_1}{c_2},\sigma_A,\mathcal{C}},g,\ctx} \nxt 
\\
\conf{\conf{c_2,\sigma_A,\mathcal{C}},g',\ctx}
\end{array}
}
{
\begin{array}{c}
g' = \gas(b,g,\sigma_A, \ctx) \geq 0
\\
\ctx,\sigma_A \models \eval{b} =\bot
\end{array}
}
$$
$$
\infer[\term{Wh}_\top]
{
\begin{array}{c}
\conf{\conf{\swhile{b}{c},\sigma_A,\mathcal{C}},g,\ctx} \nxt
\\
 \conf{\conf{c;\swhile{b}{c},\sigma_A,\mathcal{C}},g',\ctx}
\end{array}
}
{
\begin{array}{c}
g' = \gas(b,g,\sigma_A, \ctx) \geq 0
~~~
\ctx,\sigma_A \models \eval{b} =\top
\end{array}
}~~~
\infer[\term{Wh}_\bot]
{
\begin{array}{c}
\conf{\conf{\swhile{b}{c},\sigma_A,\mathcal{C}},g,\ctx} \nxt
\\
\conf{\conf{\lst,\sigma_A,\mathcal{C}},g',\ctx}
\end{array}
}
{
g' = \gas(b,g,\sigma_A, \ctx) \geq 0~~~\ctx,\sigma_A \models \eval{b} =\bot
}
$$
$$
\infer[\term{Call}]
{
\begin{array}{c}
\conf{\conf{\textit{addr}.{\textbf{call}}.\textit{value}(v).\textit{gas}(g').(f,\bar{e}),
\\
\sigma_A,\mathcal{C}},g,\ctx}
\nxt \conf{\conf{\lst,\sigma_A,\mathcal{C}}, g-g'+g'' ,\ctx''}
\end{array}
}
{
\begin{array}{c}
\ctx[\textit{addr}] = (\sigma',\textit{bal}',\mathcal{C}')~~~\mathcal{C}'.f(\bar{e}) = c
\\
g \geq g'~~~\ctx' = \ctx[\mathcal{C}.\textit{addr} \stackrel{v}{\rightarrow} \textit{addr}]
\\
\conf{\conf{c,\sigma',\mathcal{C}'}, g' ,\ctx'} \nxt \conf{\conf{\lst,\sigma_A',\mathcal{C}'}, g'' ,\ctx''}
\end{array}
}
~~~
\infer[\term{Call}_\wrong]
{
\begin{array}{c}
\conf{\conf{\textit{addr}.{\textbf{call}}.\textit{value}(v).\textit{gas}(g').(f,\bar{e}),
\\
\sigma_A,\mathcal{C}},g,\ctx}
 \nxt  \conf{\conf{\lst,\sigma_A,\mathcal{C}}, g-g'+g'' ,\ctx}
\end{array}
}
{
\begin{array}{c}
\ctx[\textit{addr}] = (\sigma',\textit{bal}',\mathcal{C}')~~~\mathcal{C}'.f(\bar{e}) = c
\\
g \geq g'~~~
\ctx' = \ctx[\mathcal{C}.\textit{addr} \stackrel{v}{\rightarrow} \textit{addr}]
\\
\conf{\conf{c,\sigma',\mathcal{C}'}, g' ,\ctx'} \nxt \conf{\conf{\wrong,\sigma_A',\mathcal{C}'}, g'' ,\ctx''}
\end{array}
}
$$
$$
\infer[\term{Tf}]
{
\begin{array}{c}
\conf{\conf{\textit{addr}.{\bf{transfer}}(v),\sigma_A,\mathcal{C}},g,\ctx} \nxt 
\\
\conf{\conf{\lst,\sigma_A,\mathcal{C}}, g-2300 + g' ,\ctx''}
\end{array}
}
{
\begin{array}{c}
\ctx[\textit{addr}] = (\sigma',\textit{bal}',\mathcal{C}')~~~g \geq 2300
\\
\mathcal{C}'.{\fback} = c~~~\ctx' = \ctx[\mathcal{C}.\textit{addr} \stackrel{v}{\rightarrow} \textit{addr}]
\\
\conf{\conf{c,\sigma',\mathcal{C}'}, 2300 ,\ctx'} \nxt \conf{\conf{\lst,\sigma'',\mathcal{C}'}, g' ,\ctx''}
\end{array}
}~~~
\infer[\term{Tf}_\wrong]
{
\begin{array}{c}
\conf{\conf{\textit{addr}.{\bf{transfer}}(v),\sigma_A,\mathcal{C}},g,\ctx} \nxt 
\\
\conf{\conf{\wrong,\sigma_A,\mathcal{C}}, g-2300 + g' ,\ctx}
\end{array}
}
{
\begin{array}{c}
\ctx[\textit{addr}] = (\sigma',\textit{bal}',\mathcal{C}')~~~g \geq 2300
\\
\mathcal{C}'.{\fback} = c~~~\ctx' = \ctx[\mathcal{C}.\textit{addr} \stackrel{v}{\rightarrow} \textit{addr}]
\\
\conf{\conf{c,\sigma',\mathcal{C}'}, 2300 ,\ctx'} \nxt \conf{\conf{\wrong,\sigma'',\mathcal{C}'}, g' ,\ctx''}
\end{array}
}
$$
$$
\infer[\term{Send}]
{
\begin{array}{c}
\conf{\conf{\textit{addr}.{\textbf{send}}.\textit{value}(v).\textit{gas}(g'),\sigma_A,\mathcal{C}},g,\ctx} \nxt 
\\
\conf{\conf{\textit{addr}.{\bf{call}}.\textit{value}(v).\textit{gas}(2300).(\fback,\emptyset),\sigma_A,\mathcal{C}}, g ,\ctx}
\end{array}
}
{}
$$
$$
\infer[\term{Dc}]
{
\begin{array}{c}
\conf{\conf{\textit{addr}.{\textbf{delegatecall}}.\textit{value}(v).\textit{gas}(g').(f,\bar{e}),
\\
\sigma_A,\mathcal{C}},g,\ctx}
\nxt \conf{\conf{\lst,\sigma_A',\mathcal{C}}, g-g'+g'' ,\ctx''}
\end{array}
}
{
\begin{array}{c}
\ctx[\textit{addr}] = (\sigma',\textit{bal}',\mathcal{C}')~~~~\mathcal{C}'.f(\bar{e}) = c
\\
g \geq g'~~\ctx' = \ctx[\mathcal{C}.\textit{addr} \stackrel{v}{\rightarrow} \textit{addr}]
\\
\conf{\conf{c,\sigma_A,\mathcal{C}'}, g' ,\ctx'} \nxt \conf{\conf{\lst,\sigma_A',\mathcal{C}'}, g'' ,\ctx''}
\end{array}
}
~~~
\infer[\term{Dc}_\wrong]
{
\begin{array}{c}
\conf{\conf{\textit{addr}.{\textbf{delegatecall}}.\textit{value}(v).\textit{gas}(g').(f,\bar{e}),
\\
\sigma_A,\mathcal{C}},g,\ctx}
 \nxt  \conf{\conf{\lst,\sigma_A,\mathcal{C}}, g-g'+g'' ,\ctx}
\end{array}
}
{
\begin{array}{c}
\ctx[\textit{addr}] = (\sigma',\textit{bal}',\mathcal{C}')~~~\mathcal{C}'.f(\bar{e}) = c
\\
g \geq g'~~~\ctx' = \ctx[\mathcal{C}.\textit{addr} \stackrel{v}{\rightarrow} \textit{addr}]
\\
\conf{\conf{c,\sigma_A,\mathcal{C}'}, g' ,\ctx'} \nxt \conf{\conf{\wrong,\sigma_A',\mathcal{C}'}, g'' ,\ctx''}
\end{array}
}
$$
\caption{Operational semantics of our Solidity core language.}\label{fig:op}
\end{figure}




